Exploring the Impacts from Datasets to Monocular Depth Estimation (MDE) Models with MineNavi

Current computer vision tasks based on deep learning require a huge amount of data with annotations for model training or testing, especially in some dense estimation tasks, such as optical flow segmentation and depth estimation. In practice, manual labeling for dense estimation tasks is very difficult or even impossible, and the scenes of the dataset are often restricted to a small range, which dramatically limits the development of the community. To overcome this deficiency, we propose a synthetic dataset generation method to obtain the expandable dataset without burdensome manual workforce. By this method, we construct a dataset called MineNavi containing video footages from first-perspective-view of the aircraft matched with accurate ground truth for depth estimation in aircraft navigation application. We also provide quantitative experiments to prove that pre-training via our MineNavi dataset can improve the performance of depth estimation model and speed up the convergence of the model on real scene data. Since the synthetic dataset has a similar effect to the real-world dataset in the training process of deep model, we also provide additional experiments with monocular depth estimation method to demonstrate the impact of various factors in our dataset such as lighting conditions and motion mode.

==> other/app.tex <==

\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.

==> other/mbl-3d.tex <==

\begin{table}[t!]
    % \caption{不同渲染器下生成数据集的精度的表现。这里使用~AbsRel~和$\delta<1.25^1$作为误差和精度指标\cite{eigen2014}，最优结果已经加粗} 
    \caption{The model shows the different accuracy results under different motion blurs}
    \label{tab:motion-blur}
    \centering
    \scalebox{0.8}{
    \begin{tabular}{l|cccc}
       \toprule[2pt] 
      & \multicolumn{3}{c}{\centering{Test Datasets}}\\
      \cline{3-3}
      \begin{tabular}[c]{@{}c@{}}Train Sets\\ (\textit{AbsRel} $\backslash\delta^1$) \end{tabular}
      & \textit{None} &\textit{low blur}&\textit{middle blur}&\textit{high blur}  \\
      \hline
      \textit{None}       &0.199$\backslash$0.768 &0.216$\backslash$0.760 &0.217$\backslash$0.758 &0.218$\backslash$0.752\\
      \textit{low blur}   &0.200$\backslash$0.730 &0.185$\backslash$0.764&0.184$\backslash$0.765 &0.186$\backslash$0.764\\
      \textit{middle blur}&0.194$\backslash$0.734 &0.177$\backslash$0.775 &0.175$\backslash$0.781  &0.176$\backslash$0.785 \\
      \textit{high blur}  &0.200$\backslash$0.730 &0.186$\backslash$0.763 &0.180$\backslash$0.774 &0.181$\backslash$0.778 \\
  
      %sildurs-10k&0.6&0.151&24&1\\
      \toprule[2pt]
    \end{tabular}
    }
    %  \vspace{-2mm}
  \end{table}
  

==> tab/mn-name.tex <==
    \begin{table}[]
        \label{tab:sub-datasets}
        \centering
        \caption{Name filed of MN dataset.}
        \scalebox{1.0}{
            \begin{tabular}{lcc}
            \toprule[2pt]
            \multicolumn{2}{c}{filed}            & value              \\ \hline
            \multicolumn{2}{c}{motion}           & mnv0, mnv1,mnv2,mnv5     \\ \hline
            \multicolumn{1}{l|}{\multirow{3}{*}{lights}} & shader & \multicolumn{1}{l}{raw, sildurs(e), sildurs(h)} \\
            \multicolumn{1}{l|}{} & motion blur  & mbl,mbm,mbh        \\
            \multicolumn{1}{l|}{} & time/weather & 6k,9k,12k,15k,rain \\ \hline
            \multicolumn{2}{c}{num}              & 2k,10k,50k            \\ 
            \toprule[2pt]
            \end{tabular}
        }
        \end{table}

==> tab/motion-blur-o.tex <==



\begin{table}[t!]
    % \caption{不同动态模糊下同一个模型表现出不同的精度结果.} 
    \caption{The model shows the different accuracy results under different motion blurs}
    \label{tab:motion-blur}
    \centering
    \scalebox{1.0}{
    \begin{tabular}{l|cccc|ccc}
       \toprule[2pt] 
      & \multicolumn{4}{c|}{Error $\downarrow$} & \multicolumn{3}{c}{Accuracy $\uparrow$}  \\
      \cline{2-8}
      motion blur  & AbsRel & SqRel & RMS & RMSlog & $<1.25$ & $<1.25^2$ & $<1.25^3$ \\\hline
      w/o blur %baseline
      &0.212&1.380&\textbf{6.217}&0.274&0.744&0.917&0.965\\
      low blur
      & 0.196 & 1.381 & 6.877 & 0.274 & 0.739 & 0.918 & 0.968 \\
      middle blur
      &\textbf{0.190}&\textbf{1.287}&6.487&\textbf{0.263}&\textbf{0.751}&\textbf{0.962}&\textbf{0.971}\\
      high blur
      &0.196&1.420&6.730&0.267&\textbf{0.751}&0.922&0.969\\


      \toprule[2pt]
    \end{tabular}
    }
    %  \vspace{-2mm}
\end{table}


